Consistent Explanations in the Face of Model Indeterminacy via Ensembling

This work addresses the challenge of providing consistent explanations for predictive models in the presence of model indeterminacy, which arises due to the existence of multiple (nearly) equally well-performing models for a given dataset and task. Despite their similar performance, such models often exhibit inconsistent or even contradictory explanations for their predictions, posing challenges to end users who rely on these models to make critical decisions. Recognizing this issue, we introduce ensemble methods as an approach to enhance the consistency of the explanations provided in these scenarios. Leveraging insights from recent work on neural network loss landscapes and mode connectivity, we devise ensemble strategies to efficiently explore the underspecification set -- the set of models with performance variations resulting solely from changes in the random seed during training. Experiments on five benchmark financial datasets reveal that ensembling can yield significant improvements when it comes to explanation similarity, and demonstrate the potential of existing ensemble methods to explore the underspecification set efficiently. Our findings highlight the importance of considering model indeterminacy when interpreting explanations and showcase the effectiveness of ensembles in enhancing the reliability of explanations in machine learning.

==> sections/future_work.tex <==
\section{Future Work}
\label{sec:future}

Compound the fact that explanations vs loss landscape analysis research exist almost in parallel. Future work includes:

\begin{itemize}
    \item Analysis across underspecification sets (rashomon set \citep{xin2022})
    \item Optimization and further analysis on perturbing weights
    \begin{itemize}
        \item Consider a selection process on the perturbations (simplest is train accuracy)
        \item Consider sampling across $\sigma$ values, since in high dimensions samples lie on a hypershell around the input (not within a hyperspherical volume)
    \end{itemize}
    \item Utilization of permutation symmetries to first align constituent models in weight space to enable faster exploration of the underspecification set. \citep{tatro2020, singh2020, ainsworth2023}
    \item Ensembling techniques: distillation, self-distillation, analysis of their effects, etc \dan{yes leonard}
    \item Perhaps the most relevant future work is combining models within the ensemble into a single point in weight space
\end{itemize}

Future work should strive to explore further properties of the loss landscape to expedite mode connectivity, building upon recent advancements in the field [REFS]. Permutation symmetries can align model weights before averaging... linear mode connectivity is possible through permutation, etc.


\paragraph{Closing remarks} convergence of neural network analysis with explanation analysis
